Cacophony: An Improved Contrastive Audio-Text Model

Despite recent advancements, audio-text models still lag behind their image-text counterparts in scale and performance. In this paper, we propose to improve both the data scale and the training procedure of audio-text contrastive models. Specifically, we craft a large-scale audio-text dataset containing 13,000 hours of text-labeled audio, using pretrained language models to process noisy text descriptions and automatic captioning to obtain text descriptions for unlabeled audio samples. We first train on audio-only data with a masked autoencoder (MAE) objective, which allows us to benefit from the scalability of unlabeled audio datasets. We then train a contrastive model with an auxiliary captioning objective with the audio encoder initialized from the MAE model. Our final model, which we name Cacophony, achieves state-of-the-art performance on audio-text retrieval tasks, and exhibits competitive results on the HEAR benchmark and other downstream tasks such as zero-shot classification.

==> tables/ablation_data_ci.tex <==
\begin{table*}[!t]
  \caption{Ablations on text preprocessing, trained on openSFX, evaluate on test split of AudioCaps and Clotho.}
  \label{tab:ab_ret}
  \centering
  \resizebox{0.75\textwidth}{!}{
  \begin{tabular}{ccccccccccccc}
    \toprule
\multirow{3}{*}{\textbf{Dataset}} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
    \cline{2-9}  & 
    \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} & \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} \\
    \cline{2-9}
    & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ && $\boldsymbol{R@10}$  $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  \\
    \midrule
    $V_1$ - $V_1$ &33.1$_{\pm1.3}$&68.8$_{\pm1.3}$&45.5$_{\pm3.1}$&76.1$_{\pm2.7}$&17.2$_{\pm1.0}$&41.2$_{\pm1.3}$&24.8$_{\pm2.6}$&51.1$_{\pm3.0}$\\
    $V_2$ - $V_1$ &32.4$_{\pm1.3}$&66.9$_{\pm1.3}$&42.7$_{\pm3.1}$&76.0$_{\pm2.7}$&15.7$_{\pm1.0}$&41.0$_{\pm1.3}$&21.5$_{\pm2.5}$&49.5$_{\pm3.0}$\\
    $V_3$ - $V_1$ &34.5$_{\pm1.3}$&67.9$_{\pm1.3}$&46.0$_{\pm3.1}$&76.1$_{\pm2.7}$&17.0$_{\pm1.0}$&42.1$_{\pm1.3}$&22.7$_{\pm2.5}$&51.1$_{\pm3.0}$\\
    $V_3$ - $V_2$ &41.6$_{\pm1.4}$&75.6$_{\pm1.2}$&55.5$_{\pm3.1}$&84.4$_{\pm2.3}$&19.9$_{\pm1.0}$&44.3$_{\pm1.3}$&24.8$_{\pm2.5}$&52.2$_{\pm3.0}$\\
    $V_3$ - $V_3$ &40.5$_{\pm1.4}$&75.2$_{\pm1.2}$&55.8$_{\pm3.1}$&83.1$_{\pm2.3}$&20.2$_{\pm1.0}$&44.4$_{\pm1.3}$&27.7$_{\pm2.6}$&53.9$_{\pm3.0}$\\
    \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/ablation_data_clotho.tex <==
\begin{table}[!t]
  \caption{Ablation study on the use of dataset for different stage training, evaluated on Clotho. $V_x$-$V_y$ represents that $V_x$ dataset is used for 1st stage MAE training and $V_y$ dataset is used for 2nd stage captioning contrastive training.}
  \label{tab:ab_ret}
  \centering
  \resizebox{0.9\columnwidth}{!}{
  \begin{tabular}{c|c|ccc|ccc}
    \toprule
\multirow{2}{*}{\textbf{Index}}&\multirow{2}{*}{\textbf{Dataset}}
& \multicolumn{3}{c|}{Text-to-Audio} & \multicolumn{3}{c}{Audio-to-Text} \\
    \cline{3-8}
    &&$\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@10}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  \\
    \hline
    (a)&$V_1$ - $V_1$ &17.2&41.2&55.2&24.8&51.2&65.8\\
    (b)&$V_2$ - $V_1$ &15.7&41.0&55.1&21.5&49.5&64.0\\
    (c)&$V_2$ - $V_2$ &18.6&42.7&56.8&25.0&52.2&66.3\\
    (d)&$V_3$ - $V_1$ &17.0&42.1&56.0&22.7&51.1&65.6\\
    (e)&$V_3$ - $V_2$ &19.9&44.3&57.3&24.8&52.2&66.1\\
    (f)&$V_3$ - $V_3$ &\textbf{20.2}&\textbf{44.4}&\textbf{57.4}&\textbf{27.7}&\textbf{52.6}&\textbf{66.8}\\
    \bottomrule
  \end{tabular}
}
\end{table}

==> tables/ablation_net_ci.tex <==
\begin{table*}[!t]
  \caption{Ablations on text preprocessing, trained on openSFX, evaluate on test split of AudioCaps and Clotho.}
  \label{tab:ab_ret}
  \centering
  \resizebox{0.75\textwidth}{!}{
  \begin{tabular}{ccccccccc}
    \toprule
\multirow{3}{*}{\textbf{Architectural design}} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
    \cline{2-9}  & 
    \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} & \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} \\
    \cline{2-9}
    & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ \\
    \midrule
    No caption head & 38.9$_{\pm1.4}$ & 73.2$_{\pm1.2}$&54.5$_{\pm3.1}$&82.0$_{\pm2.4}$& 18.7$_{\pm1.1}$& 43.0$_{\pm1.3}$& 24.7$_{\pm2.6}$& 50.4$_{\pm3.0}$\\
    PaSST audio encoder &36.4$_{\pm1.3}$ & 70.5$_{\pm1.3}$&46.7$_{\pm3.1}$&77.6$_{\pm2.6}$& 17.9$_{\pm1.1}$& 42.1$_{\pm1.3}$& 23.1$_{\pm2.5}$& 48.7$_{\pm3.0}$\\
    AudioMAE audio encoder & 40.2$_{\pm1.3}$ & 73.9$_{\pm1.2}$&55.1$_{\pm3.1}$& 82.6$_{\pm2.4}$& 19.1$_{\pm1.1}$& 43.4$_{\pm1.3}$& 25.5$_{\pm2.6}$& 53.7$_{\pm3.0}$\\
    \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/ablation_pre_text_ci.tex <==
\begin{table*}[!t]
  \caption{Ablations on text preprocessing, trained on openSFX, evaluated on test split of AudioCaps and Clotho.}
  \label{tab:ab_ret}
  \centering
  \resizebox{0.75\textwidth}{!}{
  \begin{tabular}{ccccccccc}
    \toprule
\multirow{3}{*}{\textbf{Text pre-processing}} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
    \cline{2-9}  & 
    \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} & \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} \\
    \cline{2-9}
    & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ \\
    \midrule
    None& 32.5$_{\pm1.3}$&67.5$_{\pm1.3}$&45.4$_{\pm3.1}$&76.5$_{\pm2.6}$&14.2$_{\pm0.9}$&37.2$_{\pm1.3}$&21.2$_{\pm2.4}$&51.9$_{\pm3.0}$\\
    LLM cleaning &32.6$_{\pm1.3}$&68.8$_{\pm1.3}$&45.7$_{\pm3.0}$&76.1$_{\pm2.7}$&17.2$_{\pm1.0}$&41.2$_{\pm1.3}$&24.8$_{\pm2.6}$&51.2$_{\pm3.0}$\\
    Recaptioning & 32.6$_{\pm1.3}$&66.8$_{\pm1.3}$&42.6$_{\pm3.0}$&75.6$_{\pm2.6}$&17.7$_{\pm1.0}$&43.0$_{\pm1.3}$&22.9$_{\pm2.5}$&51.8$_{\pm3.0}$\\
    \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/ablation_sam.tex <==
\begin{table*}[!t]
  \caption{Ablations on the use of SAM.}
  \label{tab:ab_sam}
  \centering
  \resizebox{0.75\textwidth}{!}{
  \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \toprule
\multirow{3}{*}{\textbf{SAM}} & \multicolumn{6}{c|}{AudioCaps} & \multicolumn{6}{c}{Clotho} \\
    \cline{2-13}  & 
    \multicolumn{3}{c|}{Text-to-Audio} & \multicolumn{3}{c|}{Audio-to-Text} & \multicolumn{3}{c|}{Text-to-Audio} & \multicolumn{3}{c}{Audio-to-Text} \\
    \cline{2-13}
    & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@10}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$& $\boldsymbol{R@10}$  \\
    \hline
    No SAM & 37.1 & 71.1&83.3&48.7&77.7&88.9& 15.5& 37.9&51.8& 19.6& 42.8&55.1\\
    $\rho$=0.025& 40.2 & 73.9&86.1&55.1& 82.6&92.1& 19.1& 43.4&57.0& 25.5& \textbf{53.7}&65.8\\
    $\rho$=0.050 & 40.5 & 74.8&85.4&54.6& 83.1&91.5& 19.3& 44.4&\textbf{58.4}& 25.9 &51.8&\textbf{66.8}\\
    $\rho$=0.075 &40.5&\textbf{75.2}&\textbf{86.7}&\textbf{55.8}&\textbf{83.1}&\textbf{92.1}&\textbf{20.2}&\textbf{44.4}&57.4&\textbf{27.7}&52.6&66.8\\
    $\rho$=0.100 & \textbf{40.9} & 74.2&85.6&54.3& 83.0&91.6& 18.6& 43.2& 58.3&25.3& 51.7&67.9\\
    \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/ablation_sam_ci.tex <==
\begin{table*}[!t]
  \caption{Ablations on text preprocessing, trained on openSFX, evaluate on test split of AudioCaps and Clotho.}
  \label{tab:ab_ret}
  \centering
  \resizebox{0.75\textwidth}{!}{
  \begin{tabular}{ccccccccc}
    \toprule
\multirow{3}{*}{\textbf{SAM}} & \multicolumn{4}{c}{AudioCaps} & \multicolumn{4}{c}{Clotho} \\
    \cline{2-9}  & 
    \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} & \multicolumn{2}{c}{Text-to-Audio} & \multicolumn{2}{c}{Audio-to-Text} \\
    \cline{2-9}
    & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ & $\boldsymbol{R@1}$ & $\boldsymbol{R@5}$ \\
    \midrule
    No SAM & 37.1$_{\pm1.3}$ & 71.1$_{\pm1.2}$&48.7$_{\pm3.2}$&77.7$_{\pm2.6}$& 15.5$_{\pm1.0}$& 37.9$_{\pm1.3}$& 19.6$_{\pm2.4}$& 42.8$_{\pm3.0}$\\
    $\rho$=0.025& 40.2$_{\pm1.3}$ & 73.9$_{\pm1.2}$&55.1$_{\pm3.1}$& 82.6$_{\pm2.4}$& 19.1$_{\pm1.1}$& 43.4$_{\pm1.3}$& 25.5$_{\pm2.6}$& 53.7$_{\pm3.0}$\\
    $\rho$=0.050 & 40.5$_{\pm1.4}$ & 74.8$_{\pm1.2}$&54.6$_{\pm3.1}$& 83.1$_{\pm2.3}$& 19.3$_{\pm1.1}$& 44.4$_{\pm1.3}$& 25.9$_{\pm2.6}$ &51.8$_{\pm3.0}$\\
    $\rho$=0.075 &40.5$_{\pm1.4}$&75.2$_{\pm1.2}$&55.8$_{\pm3.1}$&83.1$_{\pm2.3}$&20.2$_{\pm1.0}$&44.4$_{\pm1.3}$&27.7$_{\pm2.6}$&53.9$_{\pm3.0}$\\
    $\rho$=0.100 & 40.9$_{\pm1.4}$ & 74.2$_{\pm1.2}$&54.3$_{\pm3.1}$& 83.0$_{\pm2.3}$& 18.6$_{\pm1.0}$& 43.2$_{\pm1.3}$& 25.3$_{\pm2.6}$& 51.7$_{\pm3.0}$\\
    \bottomrule
  \end{tabular}
  }
\end{table*}
